Rethinking Audio-Visual Adversarial Vulnerability from Temporal and Modality Perspectives

While audio-visual learning equips models with a richer understanding of the real world by leveraging multiple sensory modalities, this integration also introduces new vulnerabilities to adversarial attacks. In this paper, we present a comprehensive study of the adversarial robustness of audio-visual models, considering both temporal and modality-specific vulnerabilities. We propose two powerful adversarial attacks: 1) a temporal invariance attack that exploits the inherent temporal redundancy across consecutive time segments and 2) a modality misalignment attack that introduces incongruence between the audio and visual modalities. These attacks are designed to thoroughly assess the robustness of audio-visual models against diverse threats. Furthermore, to defend against such attacks, we introduce a novel audio-visual adversarial training framework. This framework addresses key challenges in vanilla adversarial training by incorporating efficient adversarial perturbation crafting tailored to multi-modal data and an adversarial curriculum strategy. Extensive experiments in the Kinetics-Sounds dataset demonstrate that our proposed temporal and modality-based attacks in degrading model performance can achieve state-of-the-art performance, while our adversarial training defense largely improves the adversarial robustness as well as the adversarial training efficiency.

==> figs/attack_performance.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/pdf/av_attack_performance.pdf}
    \caption{Attack success rates of different models under different adversarial attack methods on MIT-MUSIC and Kinetics-Sounds datasets.}
    \label{fig:attack}
\end{figure*}

==> figs/defense_performance.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/pdf/defense_attack_performance.pdf}
    \caption{Attack success rates (\%) of each of $8$ deep models on the adversarial examples crafted under the white-box setting with our proposed TMA method. }
    \label{fig:defense}
\end{figure}

==> figs/draw_ens_attack_performance.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/pdf/ensemble_attack_performance.pdf}
    \caption{Attack success rates (\%) of each of $8$ deep models under the ensemble setting.  }
    \label{fig:ens_attack}
\end{figure}

==> figs/temporal_motivation.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/pdf/temoporal_motivation.pdf}
    \caption{Classification accuracy  when randomly masking $\rho$ of audio and visual frames.}
    \label{fig:tmp_motivaton}
\end{figure*}

==> tabs/attacks.tex <==
\begin{table*}[htbp]
\caption{Evaluation results of different models on the adversarial transferability. }
 \resizebox*{\linewidth}{!}{
\begin{tabular}{c|l|llllllll}
\toprule
 Datasets & Attacks & $R^{A}_{18}\mathop{-}\limits^{s}R^{V}_{18}$ & $R^{A}_{18}\mathop{-}\limits^{c}R^{V}_{18}$ & $R^{A}_{18}\mathop{-}\limits^{s}R^{V}_{34}$ & $R^{A}_{18}\mathop{-}\limits^{c}R^{V}_{34}$ & $R^{A}_{34}\mathop{-}\limits^{s}R^{V}_{18}$ & $R^{A}_{34}\mathop{-}\limits^{c}R^{V}_{18}$ & $R^{A}_{34}\mathop{-}\limits^{s}R^{V}_{34}$ & $R^{A}_{34}\mathop{-}\limits^{c}R^{V}_{34}$\\
 \hline
  \multirow{6}{*}{Music}
     & FGSM &  ~~~~~65.2& ~~~~~69.9 & ~~~~~72.4 &  ~~~~~75.6 &  ~~~~~67.0&  ~~~~~70.2 &  ~~~~~78.3& ~~~~~79.2\\
     & I-FGSM&  ~~~~~34.3& ~~~~~38.1 & ~~~~~40.3 &  ~~~~~43.7 &  ~~~~~35.7&  ~~~~~39.6&  ~~~~~45.2& ~~~~~45.7\\
     & MI-FGSM&  ~~~~~38.7& ~~~~~38.2 & ~~~~~40.8 &  ~~~~~44.1 &  ~~~~~39.1 &  ~~~~~40.3& ~~~~~47.2&~~~~~48.5\\
     & TIA&  ~~~~~76.5& ~~~~~77.1 & ~~~~~78.9 &  ~~~~~80.2&  ~~~~~77.6 &  ~~~~~78.0& ~~~~~84.5&~~~~~86.1\\
     & MAA&  ~~~~~45.9& ~~~~~46.6 & ~~~~~47.1 &  ~~~~~47.3 &  ~~~~~46.1 &  ~~~~~47.0& ~~~~~48.5&~~~~~49.2\\
     & TIA-MAA& ~~~~~82.1& ~~~~~84.3 & ~~~~~85.0 &  ~~~~~85.0 &  ~~~~~84.2 &  ~~~~~84.7 & ~~~~~87.9&~~~~~89.2\\
     \hdashline
     \multirow{6}{*}{K-S}
     & FGSM &  ~~~~~52.2 &  ~~~~~56.7 & ~~~~~62.9 &  ~~~~~64.5 &~~~~~54.1 &  ~~~~~55.8 &~~~~~68.0 &  ~~~~~70.3 \\
     & I-FGSM&   ~~~~~27.6 & ~~~~~29.5&~~~~~33.5 &  ~~~~~32.6 &~~~~~28.5 &  ~~~~~29.1 &~~~~~32.0 &  ~~~~~33.4 \\
     & MI-FGSM&    ~~~~~28.3 & ~~~~~30.2&~~~~~33.6 &  ~~~~~34.1 &~~~~~29.5 &  ~~~~~29.9 &~~~~~33.6 &  ~~~~~35.2 \\
     & TIA& ~~~~~67.5 & ~~~~~68.1&~~~~~70.2 &  ~~~~~70.3 &~~~~~68.5 &  ~~~~~68.2 &~~~~~74.5 &  ~~~~~75.3 \\
     & MAA&  ~~~~~34.4 & ~~~~~35.1 &~~~~~38.6 &  ~~~~~39.0 &~~~~~36.5 &  ~~~~~37.1 &~~~~~40.2 &  ~~~~~41.9 \\
     & TIA-MAA& ~~~~~70.8 & ~~~~~72.5&~~~~~73.7 &  ~~~~~74.2 &~~~~~73.3 &  ~~~~~73.9 &~~~~~78.3 &  ~~~~~79.0 \\
     \bottomrule
\end{tabular}}
\label{tab:attack}
\end{table*}

==> tabs/defense.tex <==
\begin{table*}[htbp]
\caption{Evaluation results of different defense methods on adversarial robustness. }
 \resizebox*{\linewidth}{!}{
\begin{tabular}{c|l|llllllll}
\toprule
 Datasets & Attacks & $R^{A}_{18}\mathop{-}\limits^{s}R^{V}_{18}$ & $R^{A}_{18}\mathop{-}\limits^{c}R^{V}_{18}$ & $R^{A}_{18}\mathop{-}\limits^{s}R^{V}_{34}$ & $R^{A}_{18}\mathop{-}\limits^{c}R^{V}_{34}$ & $R^{A}_{34}\mathop{-}\limits^{s}R^{V}_{18}$ & $R^{A}_{34}\mathop{-}\limits^{c}R^{V}_{18}$ & $R^{A}_{34}\mathop{-}\limits^{s}R^{V}_{34}$ & $R^{A}_{34}\mathop{-}\limits^{c}R^{V}_{34}$\\
 \hline
  \multirow{5}{*}{Music}
     & Ori. &  ~~~~~82.1& ~~~~~84.3 & ~~~~~85.0 &  ~~~~~85.0 &  ~~~~~84.2 &  ~~~~~84.7 & ~~~~~87.9&~~~~~89.2\\
     &Adv.Train &  ~~~~~82.1& ~~~~~84.3 & ~~~~~85.0 &  ~~~~~85.0 &  ~~~~~84.2 &  ~~~~~84.7 & ~~~~~87.9&~~~~~89.2\\
     & DCFL&  ~~~~~38.7& ~~~~~38.2 & ~~~~~40.8 &  ~~~~~44.1 &  ~~~~~39.1 &  ~~~~~40.3& ~~~~~47.2&~~~~~48.5\\
     & Mixup& ~~~~~33.9& ~~~~~32.7 & ~~~~~35.2 &  ~~~~~34.1 &  ~~~~~32.6 &  ~~~~~33.0 & ~~~~~30.8&~~~~~29.6\\
      &Ours&  ~~~~~13.4& ~~~~~15.7 & ~~~~~12.2 &  ~~~~~11.9 &  ~~~~~11.6&  ~~~~~12.0&  ~~~~~12.3& ~~~~~12.1\\
     \hdashline
     \multirow{5}{*}{K-S}
     & Ori. & ~~~~~70.8 & ~~~~~72.5&~~~~~73.7 &  ~~~~~74.2 &~~~~~73.3 &  ~~~~~73.9 &~~~~~78.3 &  ~~~~~79.0 \\
      &Adv.Train &  ~~~~~82.1& ~~~~~84.3 & ~~~~~85.0 &  ~~~~~85.0 &  ~~~~~84.2 &  ~~~~~84.7 & ~~~~~87.9&~~~~~89.2\\
     & DCFL&  ~~~~~43.9& ~~~~~44.6 & ~~~~~42.5 &  ~~~~~41.3 &  ~~~~~43.8 &  ~~~~~42.0& ~~~~~40.1&~~~~~39.9\\
     & Mixup& ~~~~~35.4& ~~~~~36.1 & ~~~~~34.2 &  ~~~~~34.9 &  ~~~~~35.3 &  ~~~~~35.8 & ~~~~~33.2&~~~~~34.0\\
      & Ours & ~~~~~15.5& ~~~~~15.5 & ~~~~~14.3 &  ~~~~~15.7 &  ~~~~~14.7 &  ~~~~~14.9 & ~~~~~13.6&~~~~~13.8\\
     \bottomrule
\end{tabular}}
\label{tab:defense}
\end{table*}
